Case law retrieval: problems, methods, challenges and evaluations in the last 20 years

Case law retrieval is the retrieval of judicial decisions relevant to a legal question. Case law retrieval comprises a significant amount of a lawyer's time, and is important to ensure accurate advice and reduce workload. We survey methods for case law retrieval from the past 20 years and outline the problems and challenges facing evaluation of case law retrieval systems going forward. Limited published work has focused on improving ranking in ad-hoc case law retrieval. But there has been significant work in other areas of case law retrieval, and legal information retrieval generally. This is likely due to legal search providers being unwilling to give up the secrets of their success to competitors. Most evaluations of case law retrieval have been undertaken on small collections and focus on related tasks such as question-answer systems or recommender systems. Work has not focused on Cranfield style evaluations and baselines of methods for case law retrieval on publicly available test collections are not present. This presents a major challenge going forward. But there are reasons to question the extent of this problem, at least in a commercial setting. Without test collections to baseline approaches it cannot be known whether methods are promising. Works by commercial legal search providers show the effectiveness of natural language systems as well as query expansion for case law retrieval. Machine learning is being applied to more and more legal search tasks, and undoubtedly this represents the future of case law retrieval.

==> literature-review/tasks.tex <==
%!TEX root = main.tex
\section{Legal research tasks}

%
% Legal information retrieval may be categorised as including the three broad tasks:
% \begin{enumerate}
% \item case law retrieval;
% \item legislation or statute retrieval;
% \item asssitive reviewing technologies for use in discovery;
% \item internal document management systems.
% \end{enumerate}
% Each of these tasks may then be further broken down.


%
% Finding Case Law on a European Scale --Current Practice and Future Work
% Van Opijnen


==> methodology.tex <==
\section{Search Methodology}

For each Jurix, for each year, went through and determined whether title was relevant. If abstract available, also judged relevancy on this too. If relevant, downloaded. 

For each JURISIN article, a relevance assessment based on the title, abstract, and keyword searches for "information retrieval" and "retrieval" was made. If not relevant, the article was not read. If relevant, the article was included for reading. Once read, a relevance assessment as to inclusion of the article was made.
2015 - Incidentally relevant, \citet{Kim_2017} and \citet{Carvalho_2017}
2013 - \citet{Kim_2014} and \citet{Tran_2014} on question and answering systems for legislation
2012 - Nothing
2011 - Nothing
2010 - Nothing
2009 - \citet{Boonchom_2010} 
2008 - Nothing
2007 - Nothing

For Artificial Intelligence and Law, relevance was first determined on the title, and then if potentially relevant, on the abstract. If relevant, then the article was included for reading. 
Vol 1 - \citet{Ashley_1992}
2 - \citet{Savoy_1993} and \citet{Soper_1993}
3 - \citet{Turtle_1995} and \citet{Smith_1995} and \citet{Lauritsen_1995}
4 - \citet{Rissland_1996} 
5 - \citet{Rissland_1997} and \citet{Saadoun_1997}
6 - \citet{Matthijssen_1998} and \citet{Uyttendaele_1998}
7 - \citet{Pietrosanti_1999} and \citet{Merkl_1999}
8 - nothing (2 relevant book reviews)
9 - \citet{Moens_2001} 
10 - nothing
11 - nothing
12 - \citet{Saias_2004}
13 - nothing
14 - nothing
15 - \citet{Peters_2007} and \citet{Schweighofer_2007} and \citet{Zarri_2007}
16 - \citet{Drumond_2008} and maybe relevant (regulation retrieval) \citet{Cheng_2008} and CBR \citet{Wyner_2008}
17 - \citet{Francesconi_2009} and \citet{Saravanan_2009} 

For JASIST, searched and then determined relevance on title, and if determined relevant, then on abstract or intro. If relevant, included. If more than 100, stopped at 100 and re-searched. 
% Queries: - "case law", "information retrieval" AND "case law" AND "law" AND "legal", legal information retrieval.

Other relevant documents included through either, citation in relevant documents or from finding by happenstance.
